Efficient Stackelberg Strategies for Finitely Repeated Games

We study Stackelberg equilibria in finitely repeated games, where the leader commits to a strategy that picks actions in each round and can be adaptive to the history of play (i.e. they commit to an algorithm). In particular, we study static repeated games with no discounting. We give efficient algorithms for finding approximate Stackelberg equilibria in this setting, along with rates of convergence depending on the time horizon $T$. In many cases, these algorithms allow the leader to do much better on average than they can in the single-round Stackelberg. We give two algorithms, one computing strategies with an optimal $\frac{1}{T}$ rate at the expense of an exponential dependence on the number of actions, and another (randomized) approach computing strategies with no dependence on the number of actions but a worse dependence on $T$ of $\frac{1}{T^{0.25}}$. Both algorithms build upon a linear program to produce simple automata leader strategies and induce corresponding automata best-responses for the follower. We complement these results by showing that approximating the Stackelberg value in three-player finite-horizon repeated games is a computationally hard problem via a reduction from balanced vertex cover.

==> changes_tobemade.tex <==
%Change the format back to single column

%New definition of GPA in the appendix

%Michal's two points

%

==> intro_new.tex <==

%Consider the following problem: $n$ people are commuting to work, and each would like to choose a route to minimize their commute time. Busier roads move more slowly, and thus the commute time of any individual is affected not only by the route they have chosen, but by the routes of the other $n-1$ people. As every player has a constant number of route choices and every commuter has an expected commute time that can be computed when all routes are fixed, the commute times can be viewed as a (perhaps quite large) payoff matrix. This is an example of a \emph{congestion game}, a game in which the payoff of selecting certain resources is affected by the choices of others. One can reason about optimal strategies and equilibria for route choices on a given day. However, the true strategy space of this game extends beyond a single daily commute. When deciding on their next route, a commuter will naturally take into account traffic patterns on previous days.  \\
%In the multi-round traffic routing game as 
%While the payoff matrix may remain static across different days, the behavior of the other commuters may not. 


%$\cdot$ Motivation for repeated games: congestion game

%$\cdot$ Current status of repeated games: no regret is very well-studied and nice
 
%$\cdot$ In zero-sum games, the standard assumption of no regret makes a lot of sense. This is because, in zero-sum repeated bimatrix games, no regret is a best response to no regret. Furthermore, the Stackelberg equilibrium in repeated games is equivalent to the stackelberg equilibrium in a one-shot game when the game is zero-sum. However, these assumptions disappear in general-sum games.


% Games model strategic interactions of rational agents, each of whom select actions which come together to decide the outcome. 
The central solution concept in games is the Nash Equilibria, where each agent is playing optimally against the mixed strategy 
of the other agents. Nash equilibria are known to always exist in finite games~\cite{nash1951non}, and the problem of computing them has been widely studied, with efficient algorithms developed for many special classes (See~\cite{nisan2007introduction}), and hardness results for general two player games (See~\cite{chen2006settling},~\cite{daskalakis2009complexity},~\cite{rubinstein2016settling}). 

% A large number of applications have led to the study of 
There are many natural variants of this problem. A solution concept of particular interest is the Stackelberg Equilibrium~\cite{Stack35}, in which one of the players, called the leader, is allowed to commit to a strategy first, and communicates this strategy to the other players. This problem was first studied through a computational lens by Conitzer and Sandholm~\cite{conitzer2006computing}, who showed efficient algorithms in the case of two players, and hardness results for three player games, and has since been the subject of many other works, including for settings such as security games (See~\cite{an2017stackelberg}). 

In another parallel line of work, repeated games have been studied as a natural generalization of the single-shot, simultaneous game --- agents repeatedly play the same game over multiple rounds, where the outcome in each round depends only upon the actions played in that round. However, a critical point of interest about these games is that the actions employed in each round may depend arbitrarily upon the history of play and the internal state of each player. In the most well-studied version of the repeated game problem, the game is played repeatedly over an infinite time horizon, with each player seeking to maximize their average payoff in the limit.

It is well-known that several phenomena arise in infinite-horizon repeated games that are not present in the single-shot setting. First, new equilibrium strategies can arise, such as cooperation in Prisoners Dilemma, a development that is generally viewed positively. Second, {\em too many} new equilibria may arise, as witnessed by the Folk Theorem, thus diluting the prescriptive power of equilibria. Third, while efficiently computing equilibria in single-shot games for even two players is a notorious open problem for which there is some evidence of intractability (\cite{rubinstein2016settling},~\cite{chen2006settling},~\cite{daskalakis2009complexity}), there is an efficient algorithm for computing Nash equilibria of two-player infinitely repeated games.

This last result was shown constructively in the work of Littman and Stone~\cite{littman2005polynomial}, who gave an efficient algorithm for computing finite automata equilibrium strategies achieving any given feasible payoff profile. In more recent work of Zhou and Tang~\cite{Zuo2015OptimalMS}, an analogous result was given for infinite repeated Stackleberg games, again providing an efficient algorithm for computing finite automata strategies (and a generalization to automata with infinite states) for both the leader and follower.  %\nat{technically they compute infinite automata strategies which can be turing computed so represetned by a turing machine... not sure if that's necessary to say here tho}

These prior works, as well as much of the literature on repeated games, seem inherently limited to the infinite-horizon setting.
%\mk{I moved the rest of this paragraph to here instead of right before the list of results, it seems like something we want to say earlier.}
Reasoning about finite-horizon games introduces many complexities not present in the infinite-horizon case. In infinite-horizon games, any finite prefix of play can be ignored, and players can have threats of unbounded length. We lose this power in finite-horizon games, and furthermore must concern ourselves with delicate order of play and ``final-round'' complexities. Despite the fundamentally different reasoning which must occur in the finite-horizon setting, we are able to show efficient algorithms for computing simple and approximately optimal Stackelberg strategies for any $T$, which are also approximately as good as any Stackelberg strategy in the infinite-horizon game.

% despite the finite-length setting being more natural and often more applicable. 
In the context of Nash equilibria, % the infinite setting is at least somewhat well-motivated; 
infinite-horizon games introduce numerous Nash equilibria which are fundamentally different from the equilibria in their finite-horizon counterparts~\cite{benoit1984finitely}. The most famous example of this phenomenon is repeated Prisoner's Dilemma, where backwards induction shows that the only finite-horizon Nash equilibrium is mutual defection at every round. By contrast, in the infinite-horizon Prisoner's Dilemma, there exist Nash equilibria where the players cooperate to achieve socially optimal payoffs. %Additionally,~\cite{halpern2014truth} show that $\varepsilon$-approximate equilibria (in the algorithm space \mk{I don't understand this comment, is it necessary?}) can be efficiently computed in the case of infinitely repeated games with constant number of players (with $poly(1/\varepsilon)$ running time), in contrast to finite-horizon games with even two players, for which the problem of finding exact NE or even $\frac{1}{T}$-approximations is known to be hard. 
% Put simply, in the case of Nash equilibria, it is often necessary to reason about infinite horizons because many equilibria are achievable solely in this setting. 

However, this is \emph{not} the case for Stackelberg equilibria; as we will see in this paper, finite-horizon repeated games give rise to Stackelberg equilibria which are comparable in power and complexity to their infinite-horizon counterparts. The nature and computation of Stackelberg equilibrium strategies in repeated games with finite horizon $T$ has previously been poorly understood. The best known results in fact appear in a related, but different line of work, which is the study of extensive-form games. The results of Letchford and Conitzer~\cite{Letchford2010} and Bosansky et al.~\cite{Bosansky2017} give algorithms to compute Stackelberg Equilibria in general extensive-form games in time polynomial and linear respectively in the size of the game tree. Since finite-horizon repeated games are a special case of extensive-form games, these results also imply algorithms to find the Stackelberg Equilibria of finite-horizon games. However, the running time guarantees are no better than exponential in $T$, since finite-horizon games cannot be succinctly represented as extensive form games. To the best of our knowledge, no prior work has explicitly focused upon Stackelberg equilibria in finite-horizon games and their algorithmic properties. % and attempted to come up with efficient algorithms to find these solutions.

In this paper, we consider algorithms for repeated Stackleberg games with finite horizon. Like previous papers on repeated games, the players in our game are allowed to employ a broad class of algorithms (essentially any finite time algorithm) to decide their strategies in each round based upon this history of play and their internal state. This allows for a large space of commitment schemes; for example, the leader can employ ``threats" such as the grim-trigger strategy in the repeated Prisoner's Dilemma. \\

\iffalse
Reasoning about finite games introduces many complexities not present in the infinite-horizon case; in infinite games, any finite prefix of play can be ignored, and players can have threats of unbounded length. We lose this power in finitely repeated games, and furthermore must concern ourselves with delicate orders of play and ``final-round'' complexities. Despite the fundamentally different reasoning which must occur in the finite-length setting, we are able to show efficient algorithms for computing simple and approximately optimal Stackelberg strategies for any $T$, which are also approximately as good as any Stackelberg strategy in the infinite length game.\\
\fi

Our main results are:
\begin{itemize}
    %\item A polynomial (in the size of the game and $T$) time algorithm for finding an approximate Stackelberg equilibrium in repeated two player games. We show that a $O(\frac{1}{T^{0.25}})$-additive~\footnote{Factor upon the size of the game\mk{I don't understand this footnote, what sentence does it modify? And is the approximation additive or a factor (multiplicative). Please clarify}} approximation to the optimal leader algorithm (Theorem~\ref{thm:stack_policy}) can be achieved by an automata for the leader (and a corresponding best-response automata for the follower). This result also features a randomized sampling scheme to construct the near optimal algorithm that is critical in obtaining the convergenece bound. We also show an algorithm that generates a leader with a  slower convergence rate that depends exponentially upon the number of actions in the game, at the advantage of an inverse linear dependence on $T$ and polynomial running time in $\log T$. These results can be found in Section~\ref{sec:main_alg}. \mk{I added mention in the abstract, but it might be good to push at least some discussion of convergence rate earlier, since it highlights a difference with the infinite horizon case. Could also break this bullet into two, one for each different algo/rate}
    %\item A convergence rate of...
    \item We give two efficient algorithms that find additively approximate Stackelberg Strategies for the leader %\mk{Again, this is not defined yet and I think we should just use "strategy" in the intro/related/techniques sections, we can be more formal when we need to} 
    that trade off different approximation factors. First, we show a $\left( \frac{2^{\text{poly}(n)}}{T}\right)$- additive approximate Stackelberg strategy where $n$ is the number of actions, which is asympotically tight in $T$. This is constructed using an algorithm that runs in polynomial time in the game size and $\log T$. We also present an approach using randomized sampling which gives a $O(\frac{1}{T^{0.25}})$-additive approximation that runs in time polynomial in the game size and $T$~\footnote{The approximation factors also depend upon the maximum number of bits needed to represent a single payoff.}. This second approach provides a slightly weaker approximation factor in $T$ in exchange for entirely avoiding dependence on $n$. Both constructions use simple automata (including states that play distributions over actions) for the leader and also for a corresponding follower best-response. We leave it as an open question whether there is an algorithm combining the best of both rates. 
    \item Building upon a reduction of Conitzer and Sandholm~\cite{conitzer2006computing} that showed that finding the Stackleberg value of a three player game is NP-hard, we show that even approximating the Stackelberg value of a three player repeated game is NP-hard (Theorem~\ref{thm:3_player_hardness}), ruling out any extension of our results for two player repeated games. We also use the same reduction to observe that approximating the Stackelberg value of three-player infinitely repeated games is NP-hard. 
    These results can be found in Section~\ref{sec:hardness_three}.
    %\item Etc.
\end{itemize}

We also show a sequence of auxiliary results, that we discuss briefly here to help the reader to navigate through the paper.

\begin{itemize}
    \item %It is not a priori clear that best responses follower algorithms are well-defined in a repeated Stackelberg game\mk{How did all these other papers on repeated Stackelberg manage to avoid the question of whether follower algos are well defined? Is this special to finite T?} We show that the Stackelberg problem is well-defined by explicitly proving their existence for finite time horizons (Lemma~\ref{lemma:bre}). Further, 
    We show that finding a follower's best-response even to a poly-time leader strategy  %(in games that admit succinct best response game playing algorithms)%
    is in general a computationally hard problem (Lemma~\ref{lemma:br_hard}). However, our approximate Stackelberg leader algorithm (Theorem~\ref{thm:stack_policy}) has an efficiently computable best-response (Lemma~\ref{lemma:br_poly}). We discuss these results in Appendix~\ref{app:br_hard}.
    \item We show that the optimal Stackelberg leader strategy %\mk{And we're also not being consistent, here we say algo instead of GPA. Let's clean this up by saying strategy everywhere up to the definition of GPA} 
    may be different from simply playing the single-shot game's Stackelberg strategy in each round of play, through the example of the well known Prisoner's Dilemma (Section~\ref{sec:separation}).
  % In contrast to some other work on repeated games(See~\cite{foster1999regret},~\cite{freund1999adaptive}), our game playing algorithms require full knowledge of the game. Many of these other works often work in an online learning setup, typically with no-regret algorithms. %, due to the many properties associated with using these algorithms to play repeated games (not least of which is the convergence of the action transcripts to (Coarse) correlated equilibria). 
    \item No-Regret algorithms are widely studied in the context of repeated games, due to their strong performance and strategic properties (See~\cite{blum2007learning},~\cite{freund1999adaptive}). A natural question is whether no-regret algorithms are in fact optimal leader algorithms in the Stackelberg setting. We show that, somewhat unsurprisingly, arbitrary no-regret algorithms are in fact Stacklberg leader algorithms in two player zero-sum games (Lemma~\ref{lemma:zs_nr_st}). %Further, we also show that any no-regret algorithm is in fact a near best response to any other no-regret algorithms in repeated two player zero-sum games. 
    In contrast, we show via a counterexample that these properties do not hold when the zero-sum condition is removed, necessitating the broadening of the search to a more general class of algorithms. These results are in Appendix~\ref{app:nr}.
    
    \item Further, we show that the class of learning algorithms (i.e. those algorithms that do not assume initial knowledge of the matrix, but learn the payoffs of each action after each round of play) does not always contain the optimal Stackelberg strategy for the leader. In (add pointer), we show a simple pricing game where learning algorithms are strictly sub-optimal for the leader to commit to.
\end{itemize}


\subsection{Our Techniques}

    In proving our main result (Theorem~\ref{thm:stack_policy}) about efficiently computing a near optimal Stackelberg leader algorithm, we use a sequence of ideas. Our main workhorse is a linear program (similar in spirit to that of~\cite{Zuo2015OptimalMS}) that is used to upper bound the average (per round) payoff that the leader can guarantee themselves against a rational follower. This linear program additionally gives us an ``ideal" empirical distribution over the action pairs that the transcript of play must follow to achieve the aforementioned value. We then convert this ideal empirical distribution into a concrete transcript of play for both the leader and follower. Akin to Littman and Stone~\cite{littman2005polynomial} and Zuo and Tang~\cite{Zuo2015OptimalMS}, we use the notion of ``threats" to stabilize such a transcript so as to force the follower to play along with it. 
    
    However, in a departure from these works, our construction carefully choreographs the order of action pairs in this transcript to ensure that the follower's best response is to follow the prescribed transcript. One might ask why we explicitly prescribe these ordered pairs, instead of allowing the leader to draw pairs from the LP distribution i.i.d. each round. The problem is that even if the leader commits to drawing from this distribution and playing their side of the strategy, they have no way to signal to the follower what they should play at any given round before play occurs. Our approach, in spirit, involves the leader pre-committing to these signals at the start of the game. However, this means that the follower can see the payoffs of the specific move pairs they will be asked to play each round (as opposed to an expected payoff over an i.i.d. draw), which necessitates the ordering of pairs by increasing follower payoff.
    The transcript we construct forces through the worst action pairs for the follower first, and adds ``treats" at the end to ensure that the follower is incentivized to follow the prescription at each round of the game. The approximation to the upper bound comes from ``fitting'' a probability distribution to a finite number of rounds $T$, and improves as $T$ grows larger. While the average values of the leader and follower in the transcript will approximate their value in the LP distribution for large $T$, the ordering means that the actual transcript will not look like a typical sequence of i.i.d. draws from the distribution.
     
    
    While the above approach gives us a rate of convergence to optimality that depends, possibly exponentially badly, on the number of actions for each player in the game, we show in Section~\ref{sec:faster} how to eliminate the dependence upon the number of actions. The main idea involved is a randomized sampling scheme that allows us to simplify the ideal empirical distribution found by the linear program. This process can also be viewed as randomized rounding of the linear program's solution to a more succinctly representable solution. This rounding also introduces randomization in the leader's algorithm, and converts the absolute guarantee of near-optimality into a high probability guarantee. %\mk{This can probably be tightened and broken into two or three paragraphs (by the way don't think we should use bullets here, just prose), but overall looks good. But I would definitely put in here the later sentence about front-loading the bad parts for the follower in exchange for better payoffs later in the sequence. We want to get across the point that our sequence will look very different than iid from the LP distribution (right?)}
    %Yes, absolutely
    
    In Theorem~\ref{thm:3_player_hardness}, where we show the hardness of approximation of computing the Stackelberg value of repeated three player games, we demonstrate a gap-producing reduction from the balanced vertex cover problem. This reduction builds upon~\cite{conitzer2006computing}, which showed that finding the Stackelberg value of three-player games is NP-hard also via reduction from balanced vertex cover. Their hard instance does not directly extend to repeated games because of the richness of new strategies available to the leader(s) in the repeated setting. Most of the work in our reduction goes into proving a stronger result about the single-shot case, which we do in Lemma~\ref{lemma:player3_min}. We can then lift this stronger result to the game with $T$ repeated rounds and prove hardness of approximation in Theorem~\ref{thm:3_player_hardness}. We also observe that the same lemma can be used to show that finding the approximate Stackelberg value of three-player infinitely repeated games is NP-hard. 
    
    %1In showing that computing best response follower algorithms is computationally hard (Lemma~\ref{lemma:br_hard}), we embed a 3-coloring instance into the repeated two player game problem.\mk{this sentence seems orphaned and unnecessary}






















% In sum, our results fill a hole in the study of repeated games by providing algorithms and hardness results for computing Stackelberg Equilibria in finitely repeated games. 

\begin{comment}

%Is the issue about the folk theorem reference?

%What is it then

%How about now?

% is this too straightforwardly saying we are similar to infinte games tho 

% also how sure are we that this result doesn't exist for nash equilibria
% I like this paragrpah but I also know there is a lot of nash research and there's a 5 percent chance the nash finite approx result does exist somewhere (or more than 5) and if this is obvious to others that would be an unforced error. so we should ask around on this. I guess Littman doesn't seem to think it exists but 

% no I like that that's fine, it's just that our approach definitely shouldnt' work for nash, not just not clearly, I think we can say. Not just because we exploit an asymmetry, but because we are implictly approximating the infinite case, which we know is impossible for nash. I think this is worth noting here. even tho we kind of said it above 

\mk{I think the next 5-6 paragraphs are largely unnecessary and should be greatly condensed and integrated above}

Ever since Nash~{} proved his seminal result showing the existence of equilibria in finite games, the concept of a Nash Equilbrium has become a topic of intense study as a predictor of the steady state of any given game. A Nash equilibrium of a game is defined as a probability distribution over strategies for each player such that no player is motivated to change their strategy, given that no other player changes their strategy.
A huge body of research has focused upon the computational problem of finding an equilibrium of a given game~\esh{Add refs}, the computational complexity of this task~\esh{Add refs}, and applications to various problem domains such as auctions, traffic networks, resource allocation, competition in markets, armament strategies, airport security etc.~\esh{Add refs}.  \mk{This first paragraph is largely unnecessary, can assume readers will be familar with basics of AGT}

A natural variant of the notion of equilibrium considers the scenario when the players do not play simultaneously as in the setting of Nash Equilibrium, but rather that one of the players, called the leader, gets to commit to their strategy in advance. The other player(s) then respond rationally to the this strategy by picking their best response. \nat{motivate why this is an importation notion of equilibria} Von Stackelberg~\esh{add ref} is one of the earliest known results that observed that the equilbria so induced in such settings (named Stackelberg Equilibria) can be markedly different from the Nash Equilbria of the same game. Conitzer and Sandholm~\cite{conitzer2006computing} showed that the Stackelberg Equilbria (SE) can in fact be computed efficiently for (single-shot) two player games.

In many real life applications of game theory such as Auctions, Congestion Games or Security Games, we are interested not just in studying a single iteration of the game once but in understanding what happens when the players repeatedly play the same game for $T$ rounds of play. For example, the same electronic auction for advertising space is repeated many thousands of times with the same set of players~\esh{add refs along with some mention of algorithms used}. Tardos et al. have analyzed empirical data of repeated auctions to see if the transcripts of play throw some light upon the underlying method used by the players to select actions in each round. Similarly, in the traffic routing problem, the same set of people drive from home to work everyday, implicitly playing the same congestion game multiple times. Blum et al.~\esh{add ref} have studied how players using no-regret algorithms in these repeated games might converge. The striking common element in these (and many other) examples is that the players employ (fairly involved) algorithms to generate strategies in each round of play, which is a significant break from single-shot games, where the players just pick a single distribution over a finite set of actions as their strategy.
\mk{Again, no need to motivate study of repeated play, assume audience familar with game theory, think entire paragraph should go}

In this paper, we are interested in the algorithms employed by the two players in a repeated bimatrix game. Nash equilibria are well-studied in such a setting; Littman and Stone~\cite{littman2005polynomial} gave a complete characterization of all possible payoffs achievable by a Nash Equilibrium of algorithms in this problem. They further showed an efficient algorithm to compute a pair of algorithms in equilibrium with each other to achieve any feasible payoff pair. The latter result served as an algorithmic analogue of the former result, a variant of which is also known as a folk theorem for repeated bimatrix games. 


However, previous work in repeated bimatrix games has thus far failed to address the Stackelberg variant of equilibrium. In a repeated Stackelberg game, instead of committing to a move distribution, the leader commits to a game playing algorithm that will output a distribution at each round according to the history of moves and random coin flips. The applications of Stackleberg equilibria naturally extend from the single-round case to the repeated games setting. \nat{say what they are }

Our paper tackles the intersection of two lines of work -- we consider the problem of computing an optimal game playing algorithm that a leader can commit to to maximize their payoff against a rational follower (who will best respond with yet another game playing algorithm). %That such a best response is well defined is not a priori obvious, requiring us to prove as such (Lemma~\ref{lemma:bre}) to set up the problem. \nat{this previous point feels like a subtlety that should be in the list below}
Our main result (Theorem~\ref{thm:stack_policy}) is to show an efficient algorithm to compute a simple, efficiently verifiable game playing algorithm that is nearly optimal for the leader to commit to. There are multiple subtleties that we want to point the reader towards regarding our main result. 
\begin{itemize}
    \item \mk{As per earlier discussion, I think this point is being overemphasized} It is not a priori clear that best responses game playing algorithms (for the follower) are well defined. We set up our problem by explicitly proving their existence for finite time horizons (Lemma~\ref{lemma:bre}). Further, we show that  finding them (in games that admit succinct best response game playing algorithms) is in general a computationally hard problem (Lemma~\ref{lemma:br_hard}). The fact that our approximate Stackelberg leader algorithm induces an efficiently computable best response (Lemma~\ref{lemma:br_poly}) is therefore a non-trivial feature of this leader algorithm.  \esh{About the verifiability} Expanding on some details, our leader algorithm also implicitly encodes a best response follower algorithm, in a form that allows the follower to verify that it is in fact a best response. We consequently use the phrase efficiently verifiable to describe the leader algorithm that we come up with for any given game.
    \item Among the space of all possible game playing algorithms, which can be arbitrarily complicated, our candidate leader $\Gpa$ \mk{I think the GPA acronym/notion should be eliminated, we should make it clear up front that strategies are arbitrary algos and our goal is to show simple, efficient algos exist} is a polynomial (in the size of the game and the number of time steps) sized automata that takes as input the sequence of play and a finite stream of random bits (similar to the automata in the results of Littman and Stone~\cite{littman2005polynomial}). Additionally, aside from explicitly showing the existence of a succinctly representable near-optimal leader algorithm, our candidate algorithm and a corresponding best response follower algorithm also each run in polynomial time to decide the action in each step. %The fact that we can efficiently construct this near-optimal leader algorithm shows the existence of succinctly representable near-optimal leader algorithms, which is also a non-trivial feature given that we define our search space to be all finite time game playing algorithms. 
    \item \mk{maybe mention briefly above, then discuss in main body} One might ask the following question -- is the optimal Stackelberg leader algorithm different from just playing the single-shot Stackelberg strategy in each round of play? We answer this question in the affirmative, through one of the simplest and well known bimatrix games, the prisoner's dilemma (Section~\ref{sec:separation}). The single-shot Stackelberg strategy in Prisoner's dilemma is to simply play defect, but we show that the optimal leader algorithm in repeated prisoner's dilemma induces action pairs other than mutual defection for a non trivial fraction of the rounds of play. Thus, committing to algorithms (rather than strategies) is one among a rich vein of settings which make action pairs other than mutual defection possible in the prisoner's dilemma (some other settings are discussed in the related work section). %\nat{technically the optimal algorithm isn't so cooperative, in fact our prisoner's dilemma section highlights a better algo which helps the leader a lot more than the follower, I'll come back and change this language in a bit}
    %\esh{Is the optimal distribution a mixture of (D,C) and (C,D)? I wonder if we can fiddle with the values to get (C,C) also in the mix. Here, C = co-op and D = Defect}
    \item \mk{condense and integrate} In contrast to some other work on repeated games(See~\cite{foster1999regret},~\cite{freund1999adaptive}), our game playing algorithms require full knowledge of the game. Many of these other works often work in an online learning setup, typically with no-regret algorithms. %, due to the many properties associated with using these algorithms to play repeated games (not least of which is the convergence of the action transcripts to (Coarse) correlated equilibria). 
    A natural question to ask is whether no-regret algorithms are in fact optimal leader algorithms in the Stackelberg setting. We show that, somewhat unsurprisingly, arbitrary no-regret algorithms are in fact Stacklberg leader algorithms in two player zero-sum games (Theorem~\ref{}). Further, we also show that any no-regret algorithm is in fact a near best response to any other no-regret algorithms in repeated two player zero-sum games. In contrast, we show via counterexample that these properties do not hold when the zero-sum condition is removed, necessitating the broadening of the search to a more general class of algorithms.
    \item \mk{leave for main body} Due to the involved nature of the set of finite time game playing algorithms, it is not clear that an optimal Stackelberg leader algorithm is well defined for repeated games (this is in contrast to single-shot games, where it is constructively shown to be well defined by the result of Conitzer and Sandholm~\cite{conitzer2006computing}). We sidestep this question, by proving a suitable upper bound for the value achieved by a leader, and show that we can get arbitrarily close to this value for a large enough $T$, the number of rounds. We also show that increasing the power of the randomization that these algorithms have access to (basically, allowing them to sample random variables from arbitrary real valued distributions) implies the existence of an optimal leader algorithm. This result is built upon making the action space for the players compact, a connection that has been observed in Proposition ?? of ~\cite{}.
    An algorithmic version of the above result remains an interesting open question.
    \item The folk theorem for Nash equilibria in repeated bimatrix games is generally viewed as a negative result \esh{cite Franklin Fisher}, since it makes a broad range of payoffs possible at equilibria, diluting the notion of Nash Equilibria as a predictive concept. The Stackelberg version of this problem stands in sharp contrast, in that our results show that any near-optimal (or optimal if any) leader algorithms in fact converge to a particular value. %\esh{Think this last point, among other things, could be written better}
\end{itemize}
 
 
In the single-shot version of this problem,~\cite{conitzer2006computing} showed that computing the Stackelberg value of a three player game is a NP-hard problem. We build upon their reduction to show that any $\frac{1}{T^{\Omega(1)}}$- additive approximation to the Stackelberg value of a repeated three player game is NP-hard (Theorem~\ref{}), ruling out an extension of our two players result to the three player setting. 
 
\subsection{Our Techniques}

In proving our main result (Theorem~\ref{thm:stack_policy}), about efficiently computing a near optimal Stackelberg leader algorithm, we use a sequence of ideas. Our main workhorse is a linear program~\esh{add ref} that is used to upper bound the average (per round) payoff that the leader can guarantee themselves against a rational follower. This linear program additionally gives us an ``ideal" empirical distribution over the action pairs that the transcript of play must follow to achieve the aforementioned value. We then convert this ideal empirical distribution into a concrete transcript of play for both the leader and follower. Akin to Littman and Stone~\cite{littman2005polynomial}, we use the notion of ``threats" to stabilize such a transcript so as to force the follower to play along with it. The approximation to the upper bound comes from ``fitting'' a probability distribution to a finite number of rounds $T$, and improves as $T$ grows larger. While our first attempt gives us a rate of convergence to optimality that depends, possibly exponentially badly, on the number of actions for each player in the game, we show in Section~\ref{sec:faster} how to eliminate the dependence upon the number of actions. The main idea involved is a sort of sampling, similar in spirit to that of Lipton et al.~\cite{}, that allows us to simplify the ideal empirical distribution spit out by the linear program. This process can also be viewed as randomized rounding of the linear program's solution to a more succinctly representable solution. This rounding also introduces randomization in the leader's algorithm, and converts the absolute guarantee of near-optimality into a high probability guarantee.

In showing that computing best response follower algorithms is computationally hard (Lemma~\ref{lemma:br_hard}), we embed a 3-coloring instance into the repeated two player game problem.

In Theorem~\ref{}, where we show the hardness of approximation of computing the Stackelberg value of repeated three player games, we demonstrate a gap-producing reduction from the balanced vertex cover problem. 

\esh{Other techniques?}

\esh{We also use a grim trigger of sorts, I think we should mention it explicitly somewhere}
\nat{yesss this was the term I was trying to remember during the meeting today!}

\end{comment}

==> outdated_files/abstract.tex <==
% We study the problem of two players playing a repeated game using algorithms to decide their strategies in each round. \nat{I understand why we use algorithm instead of policy here but it's a bit confusing to use algo to refer to the policy and then later algo to refer to how we construct the policy, not sure how to reword, thoughts? maybe we can just write policy here as we define it later down} The single round version of this problem, the standard focus of algorithmic theory, has been extensively studied, and there are a plethora of results about various types of equilibria in these games. Of particular interest to us are Stackelberg equilibria, where one of the players (the leader) gets to go first and commit to a strategy, assuming that the other player will best respond. In our primary result, we show the first algorithm to compute the approximate Stackelberg policy for a leader in the repeated game, i.e., a (near) optimal algorithm that the leader can commit to using. This result is particularly notable, given that it is not a priori clear that Stackelberg policies for repeated games are even well-defined. We show that repeated games admit a richer space of policies for the leader, and use the notion of ``threats" to construct simple, easily verifiable, near-optimal leader policies in polynomial time. We also include a brief overview of observations and results for the limited-information setting where the follower is assumed to be learning the game using a no-regret algorithm.




%We consider a novel framework of meta-games, which are repeated bimatrix games where the players use algorithms to pick moves in each round based on the history of play and results of random coin flips. While no-regret algorithms and their resulting dynamics in repeated games have been extensively studied, we turn a strategic lens upon this setting and ask about various notions of equilibria when the space of actions for each player is all possible algorithms. We observe that in these meta-games, no regret algorithms may not always be a good prediction for the behavior of rational players. In reasoning about equilibira, we therefore expand our search to the much richer class of all algorithms. Despite the complexity of the problem due the to the vast size of the search space, we show the first algorithm to compute the approximate Stackelberg equilibrium in meta-games. This result is particularly notable, given that it is not a priori clear that Stackelberg equilibria for meta-games are even well-defined. We show that meta-games admit a strictly richer space of optimal policies for the leader, and use the notion of ``threats" to construct simple, easily verifiable, near-optimal leader policies in polynomial time.

%Based on Jun 6 discussion

\begin{comment}


\mk{title: we don't need to say bimatrix. What about something a bit more crisp, like "Efficient Equilibrium Strategies for Repeated Stackleberg Games"}
We consider the problem of computing equilibria in the framework of repeated bimatrix games, where the players use algorithms to pick moves in each round based on the history of play and results of random coin flips. %While no-regret algorithms and their resulting dynamics in repeated games have been extensively studied, we turn a strategic lens upon this setting and ask about various notions of equilibria when the space of actions for each player is all possible algorithms. We observe that in these meta-games, no regret algorithms may not always be a good prediction for the behavior of rational players. In reasoning about equilibira, we therefore expand our search to the much richer class of all algorithms. 
%Despite the complexity of the problem due the to the vast size of the search space, 
We show the first algorithm to compute approximate Stackelberg equilibria in this much richer action space of algorithms. \mk{as per our last convo, I don't think we should talk about how rich the space is very much, since in the end we show simple strategies suffice. We should follow the tone of Littman and Stone in this regard} This result is particularly notable, \mk{here and elsewhere: let the reader decide whether results are notable, significant, etc.} given that it is not a priori clear that the notion of  Stackelberg equilibria is even well defined for this problem. We show that repeated games admit a strictly richer space of optimal actions for the leader (as compared to single shot simultaneous games), and use the notion of ``threats" to construct simple, efficiently verifiable (\esh{this phrase might have to be explained / replaced}), near-optimal game playing algorithms for the leader in polynomial time.

\end{comment}


 We consider the 

==> outdated_files/comments.tex <==
High level - lead with primary result -- Stackelberg in algorithm space -- add No-Regret as what ifs with zero sum games and counterexes


1. Notation for repeated games / policies
2. Simplify existence of best response proof
3. Tie to literature about when cooperation is possible in prisoner's dilemma...Axelrod, Bounded rationality, uncertain time horizon
4. Outline for the algorithm and proof at the beginning of Sec 3
5. Simplify LP upper bound, mainly notation, if possible
6. Threat Value --> Safety Value
7. Highlight ordering is important while constructing the recommended transcript -- simple counterexample possibly --> Prisoner's dilemma --> Contrast to no-regret (there is an underlying exchangeability that is being exploited)
8. Rational entries? --- Truncation of irrational nos. preserves equilibria with approximation -- if so, we can prove and remove the assumption that entries have to be rational
9. L&S --- what did they do about finite time horizons?
10. Lower bounds for the approximation factors --- algorithm specific? More general proof?
11. Rewrite the AN dependence in terms of natural quantities
12. Push the sampling idea to the outline
13. In case L&S does not deal with finite -- let's fix that gap for them in an appendix
14. Expository point about the folk thm. non equivalence - no longer almost anything that can happen -- no longer multiple values --- no more folk thm. when thinking of Stackelberg-- known conceptually beforehand possibly, made concrete here.


Jun 16

1. Commit to automata
2. Tie closer to L&S
3. Infinite game -- can adapt-- but issues with best response, algorithm size..
4. Table comparing L&S, Conitzer, us 


==> outdated_files/intro.tex <==




%Filler text about Nash equilibria
Ever since Nash~{} proved his seminal result showing the existence of equilibria in finite games, the concept of a Nash Equilbrium has become a topic of intense study as a predictor of the steady state of any given game. A Nash equilibrium of a game is defined as a probability distribution over strategies for each player such that no player is motivated to change their strategy, given that no other player changes their strategy.
A huge body of research has focused upon the computational problem of finding an equilibrium of a given game~\esh{Add refs}, the computational complexity of this task~\esh{Add refs}, and applications to various problem domains such as auctions, traffic networks, resource allocation, competition in markets, armament strategies, airport security etc.~\esh{Add refs}.  

%Text about Stackelberg Equilibria

A natural variant of the notion of equilibrium considers the scenario when the players do not play simultaneously as in the setting of Nash Equilibrium, but rather that one of the players, called the leader, gets to commit to their strategy in advance. The other player(s) then respond rationally to the this strategy by picking their best response. Von Stackelberg~\esh{add ref} is one of the earliest known results that observed that the equilbria so induced in such settings (named Stackelberg Equilibria) can be markedly different from the Nash Equilbria of the same game. Conitzer and Sandholm~\cite{conitzer2006computing} showed that the Stackelberg Equilbria can in fact be computed efficiently for two player games.

In many real life applications of game theory such as Auctions, Routing Games or Security Games, we are interested not just in studying a single iteration of the game once but in understanding what happens when the players repeatedly play the same game for $T$ rounds of play. While Nash/ Stackelberg equilibria are a natural predictive concept for the steady state of a single round game, they may not continue to play the same role when the players know beforehand that they will be playing the same game for multiple rounds. In this new setting, each player's action space now expands to all algorithms that observe the play in previous rounds and generate strategies for the next round, which we refer to as \emph{policies}. Thus, these repeated games can be thought of as {\bf meta-games} where the players have the set of all possible (strategy generating) algorithms as their action space. Indeed, this meta-game setting has been the object of study of multiple papers that attempt to characterize the policies used by players in such a setting. Notable works in this space include~{(Littman and Stone, Deng at al., Syrgkanis et al.) }. The meta-game problem has also been studied in the context of learning where one or more of the players start out with little to no information about the game (i.e. the payoff matrices) and actively learn the game using the information they get in each round of play while trying to maximize their payoffs.  

Our {\bf main technical result} is to extend the notion of Stackelberg Equilibria to the meta-game. We show the first efficient algorithm for finding a near-optimal Stackelberg policy in a two player Stackelberg meta-game. We also present a unified picture of the two prominent lines of work in the meta-game space. 

We focus upon two distinct lines of investigation into these classes of games. 
In the first line of investigation, one of the players is assumed to not have full information about the payoff matrices. One natural class of algorithms to consider in this setting is No Swap Regret algorithms, and we assume that Player 2 is playing some algorithm from this class. No Swap Regret algorithms only learn the payoff matrix by observing the columns associated with their moves each round, but still have strong guarantees on the gap between expected payoff and the payoff of the best swap strategy.

It is particularly interesting to reason about when Player 1 might commit to a policy with No Swap Regret guarantees when Player 2 is restricted to playing No Swap Regret algorithms. When both players play No Swap Regret in a repeated game, the historical average strategies for each player form an approximate Nash Equilibrium (for zero-sum) or Correlated Equilibrium (for general-sum) for the underlying game ~\cite{freund1999adaptive}. Thus, in cases where No Swap Regret is a best response against No Swap Regret, the equilibria of the game will be computed as a byproduct of strategic play.


In the second line, propounded by Littman and Stone~\cite{littman2005polynomial} for two player games, the players are assumed to know the entire matrix beforehand. For this setting, \cite{littman2005polynomial} showed the existence of a succinct representation of the set of all possible payoffs induced by an equilibria in the meta-game and also gave a polynomial time algorithm to find a pair of policies that induce any particular feasible payoff pair. Further, their characterization also constructively showed the existence of a Nash Equilibrium in this meta-game. %NOTE[Natalie]: don't they \textbf{explicitly} show the existence via construction? Esh - good point, fixed it
\nat{Should make this description at least as long as the learning setting description, as it's the result we want to emphasize.}

\subsection{Our Results}
Our central question of interest asks what the optimal policy is for Player 1 to commit to in this meta-game setting. Such a policy can be thought of as a meta-game analogue of the Stackelberg strategies introduced and studied by Conitzer and Sandholm~\cite{conitzer2006computing}.

 We consider two cases: where Player 2 is a no-regret learner, and where Player 2 has full information about the game and the algorithm of Player 1, as well as unbounded computational resources to generate an optimal policy in response.  The latter is the central problem that we investigate in this paper, and in the table below, we present an overview of the results known about optimal policies for two player games in these two settings in Table. 
\\
\\
\\



In the first row, we consider the special class of two player zero-sum games. When Player 2 is playing a No Swap Regret Algorithm, Player 1 can in fact do no better in the limit (as $T \rightarrow \infty$) than responding with a No Swap Regret Algorithm of their own. Furthermore, in the full information setting for Player 2, committing to playing a No Swap Regret Algorithm is an optimal strategy (again, in the limit) for Player 1. While these results are already generally known, we present them explicitly and situate them in the broader meta-game context. Tardos~\esh{add ref} mentions that there also exist best responses to No Swap Regret algorithms that are \emph{not} No Swap Regret algorithms; in our results, we include such a counterexample. 

In general sum games, one might ask if it is still near-optimal for Player 1 to commit to No-Regret against a Player 2 who plays a No-Regret Algorithm. However, we show, through a counterexample, that this is not necessarily the case~\esh{Add ref}. The result of Deng at al.~\cite{deng2019strategizing} showed that the Stackleberg value of the single round game is essentially the optimal value of any policy played against a learner playing a No (Swap) Regret Algorithm. Interestingly, this is also the optimal value obtained by Player 1 committing a policy in the single round version of the game when Player 2 has full information about the game and Player 1's policy. In both settings, the optimal policy of Player 1 is to repeatedly play the single round Stackelberg policy, or a small variation thereof.  \nat{Might wanna move this below the next paragraph. If we are going to start with best-responding followers in the paper, we should start with best-responding followers in this paper outline.}

Our main technical result is motivated by the observation that this is not necessarily the optimal Stackelberg policy in the multi round setting when Player 2 has full information. Indeed, a simple example involving a variant of the Prisonner's Dilemma suffices to illustrate this point~\esh{Add ref}. We use a Linear Programming based method to efficiently construct a policy for Player 1 that is approximately optimal to commit to , with the approximation factor improving with increasing time horizon. Our methods also feature using ``threats" to stabilize certain types of equilibria, which is an idea that features prominently in the results of Littman and Stone~\cite{littman2005polynomial}. This result, and the accompanying technique, are quite surprising, given the complex space of policy pairs. In order to find the optimal policy, we potentially need to search through the space of all policies, and for each, reason about the best response policy by the follower. In fact, it is not even obvious a priori that a best response to a policy is well-defined.%. %\esh{We may have to reconsider this statement}. 
By contrast, to find a Stackelberg strategy in a single-round game by brute force, one would only need to search through the space of all mixed strategies, and reasoning about the best response by the follower to each mixed strategy is trivial. However, while computing a Stackelberg in a single-round game requires multiple linear programs, one for each pure action of the responding player, we only need to solve an auxiliary linear program and search through a suitably constructed polytope to find an optimal policy in the meta-game setting. Additionally, we use independent sampling to modify our candidate policy so as to make the approximation factor independent of the number of actions available to the two players.




==> outdated_files/sampling.tex <==
\subsection{Randomization for Faster Convergence}

We complete the proof of the theorem by showing that the judicious use of randomization can guarantee faster convergence, independent of the number of actions $n$, to optimality. In our current candidate policy, the rate of convergence to optimality depends upon the number $N$, which is the least common multiple of the denominators of the probabilities associated with each action pair. Since each probability can take polynomial in $n$ and $b$ (i.e. polynomial in the size of the game) bits to write down, these denominators can be exponentially large in $n$. However, since we are already working with an approximation, one might ask if probabilities with large denominators can be approximated by a rational number with a more tractable denominator without significant loss in the  objective and maintaining the constraints. In other words, we would like to round our LP solution to more tractable fractions. Randomized Sampling serves us well in this exercise -- replacing the probability distribution $\alpha$ by the empirical average of a sufficiently large number of samples allows us to use standard concentration inequalities to approximate the optimum as well as the constraints with high probability (since both of these are linear functions of the probability distribution). \nat{unsure if we should think about both of them as constraints. really there's just one constraint (incentive compatibility for the follower), which we need to always satisfy, and one objective, which we need to approximately satisfy} Tweaking the resulting distribution slightly to exactly satisfy the constraint suffices to build a new probability distribution with a smaller cycle length. In particular, this cycle length only depends on the number of samples which in turn is independent of $n$, the number of actions, for any target approximation value. 

The empirical distribution $\al$ over action pairs is constructed by drawing $\ell$ I.I.D samples $a_1, a_2 \cdots a_\ell$ from $\alpha$ and taking the uniform distribution over them where $\ell := \frac{100}{\varepsilon^2}$ for some approximation factor $\varepsilon > 0$ (we will specify $\varepsilon$ at a later stage when it is convenient for us). Using the Hoeffding bound along with an application of the union bound, the following two inequalities hold with probability at least $0.99$

\begin{align*}
    \lpopt - \frac{1}{\ell} \sum_k M_1(a_k) &\le A \cdot \varepsilon \\
    V - \frac{1}{\ell} \sum_k M_2(a_k) &\le A \cdot \varepsilon
\end{align*}

\esh{Need to explain by pointing out the R.V.s that we are using the Hoeffding bound over}

While the first inequality adds to the distance from optimality, the second inequality is a more serious matter. This is because the threat offered by the leader is only credible if the prescribed transcript offers something no worse than the threat value. In particular, if we already have $V' := \frac{1}{\ell} \sum_k M_2(a_k) \ge V$, then we have nothing to worry about. However, the other case demands some modifications to $\al$. In this event, $\al$ is tweaked by mixing it with a treat to ensure that the expected payoff for the follower from $\al$ is at least $V$. Let $(m_1,m_2)$ be one of the action pairs that generates maximum possible value for the follower. The final distribution $\al'$ is then constructed as :

\[ 
\al' := \begin{cases}
\alpha \text{ with probability } 1- \delta \\
(m_1,m_2) \text{ with probability } \delta 
\end{cases}
\]

i.e., we re-normalize $\alpha$ so that the probabilities add up to $1-\delta$ and put the remaining mass on the action pair $(m_1,m_2)$. We will choose $\delta > 0$ so as to ensure that the expected payoff of the follower is at least $V$. Recall that we use $m$ to denote the maximum possible payoff of the follower. Enforcing this condition gives us $\delta \ge \frac{V-V'}{m-V'}$. As a sanity check, since $m \ge V$, we get $\delta \le 1$. Further, unless $m = V$, we know that $\delta < 1$ ~\footnote{The case of $m=V$ is a somewhat special case, in essence, the leader already knows that the follower will settle for nothing less than $m$ and will therefore repeatedly play one half of the action pair that maximizes the leader's payoff subject to getting the follower $m$.}. On first glance, it appears intuitive that we pick the smallest possible value of $\delta$ so as to guarantee proximity to optimality.%, so we set $\delta  = \frac{V-V'}{m-V'} = \frac{1}{\frac{m-V'}{V-V'}}$
~\esh{Note to self : In this step, push up $\delta$ to be a multiple of the smallest possible difference/ lcm of the payoff matrix denominators}. 
However, such a choice of $\delta$ might have a downside -- in that, this particular value could be very fine-grained, taking polynomial in $n$ bits to write down. Consequently, the probabilities of action pairs in $\al'$ could also be fine-grained, resulting in large cycle lengths (exponential in $n$) and thus invalidating the attempt to have cycle lengths with a better dependence upon $n$, the number of actions. Taking a deeper look into the quantity $\frac{V-V'}{m-V'}$, there are three variables of interest- $V$, $V'$ and $m$. $m$ is no more fine-grained than $A$, by definition. Further, $V'$ can also be described in terms of $A$ and $\frac{1}{\varepsilon^2}$. The problem lies with the threat value $V$, which is the result of a linear program and can be exponentially fine-grained in $n$. {\it Our fix for this problem is to round $V$ up to $V^*$, the nearest multiple of $1/A$}. First of all, this should preserve $\delta \le 1$. Since $\frac{V-V'}{m-V'} = 1$ occurs only when $V = m$, we do not have to do anything special to deal with this case (since $V$'s bit complexity does not depend upon $n$). For any other case, the definition of $A$ guarantees that $V^* \le m$ and hence $\delta  = \frac{V^*-V'}{m-V'} \le 1$. %We can now rewrite $\delta$ as $\frac{1}{\frac{m-V'}{V^*-V'}}$ and get the crucial guarantee that the denominator is at most $\frac{100 A^2}{\varepsilon^2}$. 
Thus, if we use the same procedure in the previous subsection to construct a policy $\pol^*(\al')$ based on $\al'$, the cycle length of this policy is upper bounded by $\frac{100}{\varepsilon^2 \delta}$.

Finally, we work out the additive approximation to $\lpopt$. The average payoff guaranteed to the leader by $\al'$ is at least $(1-\delta)(\lpopt - A \varepsilon) + \delta m'$ where $m'$ is the leader payoff for the action pair $(m_1,m_2)$.

\begin{align*}
    \text{Leader Payoff } &=  (1-\delta)(\lpopt - A \varepsilon) + \delta m' \\
    &= (1-\delta)(\lpopt - A \varepsilon) + \delta m' + \delta \lpopt - \delta \lpopt \\
    &= \lpopt - (1-\delta) A \varepsilon - \delta (\lpopt -m') \\ 
    &\ge \lpopt - (1-\delta) 
    A \varepsilon - 2\delta A %xs\\
      % & = \lpopt - A \varepsilon - 2 A \frac{V^*-V'}{m-V'}\\
   % &\ge \lpopt - A\varepsilon - 2 A  \text{ (since $\delta \le 1$ --- not a good approx!!) } \\
    %&\ge \lpopt - A \varepsilon - 2 \frac{A^3}{ \varepsilon} \\
    %&\ge \lpopt - 3 A
\end{align*}

Additionally, when we construct a policy $\pol^*(\al')$, we take a further loss of $A \cdot N(\al') $ where $N(\al')$ is the cycle length of $\al'$, thus this total loss is upper bounded by $\frac{100 A}{\varepsilon^2 \delta}$, and the average loss by $\frac{10000 A^3}{\varepsilon^4 T}$. Thus the total approximation to $\lpopt$ is $A \varepsilon + 2 \delta A + \frac{100 A}{\varepsilon^2 \delta}$.
\esh{Stuck here, but I think the fix is to consider various values of $\delta$ between the upper and lower bounds...}%\esh{Too lax! Wait for this to be fixed before reading} %Selecting $\varepsilon = \theta (\frac{1}{T^{1/3}})$ minimizes this quantity, giving us an additive approximation factor of $\frac{A^3}{T^{1/3}}$.

==> outdated_files/stackelberg.tex <==
Outline --

\begin{enumerate}
    \item   Set up the problem -- what is a Stackelberg policy setup -- A sequence of functions, of increasing arity
    \item Separation between repeating static Stackelberg strategy T times
    \[ \begin{bmatrix}
(C,\epsilon) & (0,1+\epsilon) \\
(0,0) & (0, 0)
\end{bmatrix} \]
Here, $C$ and $\epsilon$ are both values strictly larger than $0$.
If player $1$ is the leader, the stackleberg equilibrium gives them a payoff of $0$. 

    \item Describe the candidate algorithm - LP and Rounding to construct a T round policy
    \item Proof of Optimality
\end{enumerate}


\subsection{Preliminaries}
We study a bimatrix game between two players - a leader and a follower each having the same number $n$ of actions- that is played repeatedly for $T$ rounds. For each player, the maximum difference in the payoff of any two outcomes is assumed to be $1$. Each player submits a policy at the beginning that plays on their behalf. A policy consists of $T$ functions (we assume that both players have access to the payoff matrices and thus these functions can be chosen based upon the payoff matrices) -one for each round. The function $f_t$ for the $t$-th round takes as input the actions played by both players in the first $t-1$ rounds and outputs a distribution over the $n$ actions to be played in the $t$-th round, i.e., $f_t : [n]^{2(t-1)} \rightarrow \Delta^n$.

In the single round game (alternatively referred to as the static setting), the notion of a Stackelberg strategy is well defined-- the leader picks a distribution $x^* \in \Delta^n$ and the follower plays some pure strategy $e_j$ that is a best response to $x^*$ (where $e_j$ represents the $j$-th standard basis vector in $\mathbb{R}^n$, which in turn corresponds to the pure strategy that picks the $j$-th action). The choice of $x^*$ seeks to maximize the payoff of the leader in such a setting. In other words, the Stackelberg strategy and the induced Stackelberg equilibrium captures what a rational player would commit to knowing that the other player will respond rationally. Conitzer and Sandholm~\cite{conitzer2006computing} showed how to efficiently compute a Stackelberg policy using the best of $n$ linear programs. We generalize the notion of a Stackelberg equilibrium for $T$ round repeated bimatrix games. In our setup, the leader commits to a policy $\cL^*$, seeing which the follower comes up with some policy $\cF$ that is a best response (\esh{Bit worried that this may not be a well defined object -- think we should be able to get around this by allowing $\varepsilon$ approximate BRs for arbitrarily small $\varepsilon$ - alternatively, if we can bound the size of the policy --akin to some bounded rationality business-- then the best response is well defined since we would have a finite set to search over - for instance, we can limit the size of the Turing Machine used to compute each round's strategy}). 
% \subsection{Separation from Single-Round Stackleberg}

%A natural question to ask is whether the $T$ round Stackelberg policy is just the static Stackelberg strategy $x^*$ repeated for $T$ rounds. In fact, the leader can leverage the multiple rounds of play to perform arbitrarily better on average than they do in static Stackleberg. The following bimatrix game shows a clear separation between the Stackelberg policy and repeating the static Stackelberg strategy. 

% \[ \begin{bmatrix}
% (C,1) & (0,1+\epsilon) \\
% (0,0) & (0, 0)
% \end{bmatrix} \]

%We set the row player to be the leader and the column player to be the follower. Further, we have $C, \varepsilon > 0$. The static Stackelberg equilibrium of this game gives the leader the value 0, since if the leader puts any weight on row 1, the follower must play row 2 and the leader gets a payoff of 0 if he plays row 2 or the follower plays column 2. We exhibit another policy for the leader that guarantees a payoff of at least $C(T-1)$ -- the row player (the leader) always plays row 1 until the column player plays column 2, at which point, the row player switches to always playing row 2. We claim that the column player's best response policy is to play column 1 for the first $T-1$ rounds and play column 2 in the last round. This nets the column player a payoff of $T + \varepsilon$. Consider any other policy for the column player against the posted policy of the row player. If the induced transcript never has the possibility of playing column 2, the payoff to the column player is upper bounded by $T$ and is hence not a best response. Consider any policy that results in column 2 being played for the first time in round $t$ (this might happen with some probability between $0$ and $1$, but the analysis will still hold). The resulting payoff for the second player in such an event is upper bounded by $t-1 + (1+\varepsilon) = t + \varepsilon$. Thus, if $t<T$, this policy is also sub-optimal, which completes the proof of our claim. Under this best response, the payoff of the leader is $C(T-1)$, which is arbitrarily better than the payoff of repeating the static Stackelberg strategy (since $C$ can be made as large as desired).\\

%We have now established that the repeated game Stackelberg policy is no simple extension of the static Stackleberg strategy. Furthermore, this example gives us some intuition for what good leader policies might look like in general. The leader was able to leverage a threat (playing row 2 for the remainder of the game) in order to force the follower to obey a specific move sequence (follower plays column 1, leader plays row 1). Actually implementing this threat would give the leader minimal payoff along with the follower. But the best-responding follower does better by obeying the leader than by being exposed to the threat, so they will play along. The threat will therefore never be implemented, and the leader is free to reap the rewards of the intended sequence. \\
\\
%

\subsection{Main Result}
% We now state and prove the main result of this section, which shows an efficient algorithm to construct the Stackelberg policy when $T$ is either a multiple of a natural number that depends on the game, or in the limit as $T$ approaches infinity. We begin by describing an LP for any bimatrix game which upper bounds the value of the best Stackleberg policy for any $T$. Then, we describe a way to construct a policy using the LP output such that a best response by the follower results in a leader payoff closely approximating the LP value. 

% \begin{theorem}
% There exists an efficient algorithm to compute an approximate Stackelberg policy of a given bimatrix game that is repeated for $T$ rounds, further the computed policy becomes optimal as $T \rightarrow \infty$. 
% \end{theorem}


% \subsubsection{An LP Upper Bound}

% We describe the construction of the linear program for any bimatrix game. First, we precompute the ``threat" value $V$ of the column player along with the associated strategy for the row player $x^*$, which we call the threat strategy. This is defined as the minimum payoff that the column player can receive by best responding to the row player's strategy in the static setting i.e. $V : = \min_{x \in \Delta^n} \max_j x^\intercal B e_j $ where $B$ is the payoff matrix of the column player. Note that this is equal to the value of a hypothetical zero sum game between the two players where the row player's payoff is changed to be the negative of the payoff of the column player, and can hence be computed in polynomial time, as can the associated strategy $x^*$ of the row player. The reason we call this the threat value is that the row player could find a strategy that ensures the column player can do no better than $V$ against this strategy in any given round of play.

% Next, we compute the solution of a linear program whose variables are weights $\{\alpha_{i,j}\}_{i,j}$ attached to each action pair in $\{i,j\}^2$. Intuitively, the point of the linear program is to find a prescribed distribution over the action pairs that maximizes the payoff of the leader subject to the follower receiving at least their threat value. Here $u^1$ and $u^2$ represent the payoff matrices of the leader and follower respectively.

% \begin{flalign*}
%     \max \sum_{i,j} u^1_{i,j} \alpha_{i,j} \qquad \qquad  \alpha \in \mathbb{R}^n &\\
%     \text{ subject to } &\\
%     \sum_{i,j} u^2_{i,j} \alpha_{i,j} \ge V &\\
%      \sum_{i,j} \alpha_{i,j} = 1 &\\
%     \alpha_{i,j} \ge 0 \qquad \qquad \text{ for } i,j \in [n]^2 &
% \end{flalign*}

% The intuition behind the candidate Stackelberg policy is as follows -- the leader prescribes a sequence $\cA = a_1, a_2, \cdots a_T$ of action pairs for both leader and follower to adhere to. In case the follower ever deviates from this prescribed sequence, the leader then plays the threat strategy $x^*$ for the remaining rounds. This sequence is built based upon the LP solution $\alpha$ and has two key properties -- first, that the empirical distribution over action pairs in this sequence approximates the distribution $\alpha$ and second, that at any point in the sequence, the follower never gains more by deviating from the sequence than following it. 


% We observe that the above LP is feasible. In particular, the distribution over action pairs induced by the threat strategy $x^*$ of the leader and the best response of the follower is by construction a feasible point. Additionally, since the objective describes the payoff generated for the leader by some distribution over the action pairs, the LP is bounded above by the maximum payoff of the leader in the game. Consequently, the LP has a well defined optimum.

% \begin{lemma}
% \label{lemma:lp_upper_bd}
% The optimum value $\opt$ of the LP upper bounds the expected per-round payoff of a Stackleberg policy for any $T$.
% \end{lemma}



% \begin{proof}
% For some bimatrix game $M$, let the value of the above LP be $OPT_{LP}$. 

% Assume for contradiction that for $M$, there exists a policy $L^{*}$ that the leader can declare such that, when the follower best responds, the expected leader payoff is $OPT > OPT_{LP}$. Just like the leader's policy, the follower's policy can be described as $T$ different functions, where the $t$th function takes as input the transcript of play of length $t-1$ and outputs a probability distribution over pure actions to play in round $t$. So the follower will respond to $L^{*}$ some policy $F^{*}$. Reasoning about the precise behavior of these policies in tandem might be complex--both policies could be randomized and could be sensitive to different realizations of their or their opponent's randomness. But, when played in tandem, $(L^{*}, F^{*})$ will always produce an output which is a sequence of $T$ move pairs. Furthermore, this sequence is determined only by the declared policies and the coin flips of each player. Therefore, $(L^{*}, F^{*})$ induces a distribution $D^{*}$ over sequence outcomes. \\

% We can think of $D^{*}$ as a vector of all possible $T$-length move pair sequences. $D^{*}_{i}$ is the weight in the distribution placed upon the $i$th sequence (for some arbitrary indexing of sequences). For any sequence of move pairs $s$, let $v_{1}(s)$ be the total payoff of the leader, and let $v_{2}(s)$ be the total payoff of the follower. So, the expected payoff per round for the Leader under $D^{*}$ is
% $$OPT = \frac{1}{T} \sum_{\forall i \in S}v_{1}(D^{*}_{i})\cdot P(S = i)$$

% As $D^{*}_{i}$ is just some particular sequence of (not necessarily unique) move pairs $x_{i1},...,x_{iT}$, we can rewrite this as

% $$OPT = \frac{1}{T}\sum_{\forall s \in S}\sum_{t=1}^{T} u^{1}(x_{st})\cdot P(S = s)$$

% Note that the $x_{st}$'s are not necessarily unique, as a move pair can appear with some probability at different rounds and in different sequences. We can rewrite this with respect to each unique move pair, which we will call $(i,j)$:

% $$OPT = \frac{1}{T}\sum_{t=1}^{T} (\sum_{\forall i,j}(u^{1}_{i,j}\cdot \sum_{\forall s \in S}P(S = s, s[t] = (i,j))))$$

% Note that for a particular time $t$, $\sum_{\forall i,j} \sum_{\forall s \in S}P(S = s, S[t] = (i,j)) = 1$. Therefore, for every fixed time $t$, there is a probability distribution over all move pairs. $OPT$ is simply the sum of $T$ different distributions over move pairs, divided by $T$. So OPT can also be seen as $u^{1}$ applied to some distribution over move pairs. \\

% NOTE[Natalie]: I don't like how I wrote this, this can be made much simpler and intuitive, TODO.\\

% Thus, we know that there exists some distribution over move pairs $\alpha$ such that
% $$OPT = \sum_{i,j}u^{1}_{i,j}\alpha_{i,j}$$

% Using the same logic as above, just swapping $v_{2}$ for $v_{1}$, the value that the follower gets in this game, which we will call $OPT_{F|L}$, can be written as 
% $$OPT_{F|L} =  \sum_{i,j}u^{2}_{i,j}\alpha_{i,j}$$
% As the follower is best-responding, it must be the case that $OPT_{F|L} \geq V$. By definition, the follower can always guarantee themselves $V$ each round, so if this were not the case, the follower would not be best-responding. So, we have some distribution over move pairs $\alpha$ such that 
% $$\cdot \sum_{i,j}u^{1}_{i,j}\alpha_{i,j} = OPT > OPT_{LP}$$
% $$\cdot \sum_{i,j}u^{2}_{i,j}\alpha_{i,j} \geq V$$
% $$\sum_{i,j}\alpha_{i,j}=1$$
% $$\alpha_{i,j} \geq 0$$

% Thus, $\alpha$ is a valid solution to the LP described previously, and the objective is larger than $OPT_{LP}$. But we assumed at the start of this proof that $OPT_{LP}$ is the optimal solution to the LP. Therefore we have derived a contradiction, and there cannot exist a Stackleberg policy $L^{*}$ that garners expected payoff above $OPT_{LP}$.


% \end{proof}


% \subsubsection{Construction of a Stackelberg Policy from the LP}

% The above LP solution gives us the optimal distribution over action pairs that the follower would be incentivized to play. If the leader and follower had a shared source of randomness, they could draw from this joint distribution each round and preserve both optimality for the leader and incentive compatibility for the follower. However, in our setting, there is no shared source of randomness. Therefore in our policy the leader will prescribe a $T$-round sequence inspired by the LP solution, which preserves incentive compatibility while approximating optimality.

% To aid with explicitly describing this sequence, we introduce some notation. We know that there is a polynomial time algorithm for solving a linear program with rational coefficients that outputs a rational solution. Our linear program has all coefficients rational -- the only non trivial observation is that the threat value $V$ is also a rational number (we are assuming that the payoff matrix of the column player (the follower) is rational), since it is itself the optimum of a linear program with rational coefficients. Therefore, we can assume that each $\alpha_{i,j}$ can be written in canonical form as $\frac{p_{i,j}}{q_{i,j}}$ where $p_{i,j},q_{i,j} \in \mathbb{N}$. For the next step, we re-index the action pairs from $1$ to $n^2$ such that for any two action pair $k_1,k_2 \in [n^2]$ with $k_1 < k_2$, we have $u^2[k_1] \le u^2[k_2] $. We use this indexing for the action pairs henceforth. Let $N = LCM(q_1,q_2 \cdots q_{n^2})$ and let $T = c \cdot N + r$ where $c$ is a natural number and $r \in \{0,1,2,\cdots N-1\}$. We assume $T$ is large enough to ensure $c \ge 1$. 

% For each action pair $k$, we calculate the number of times $n_k$ to prescribe playing this action pair in the first $c \cdot N$ rounds, $n_k := \alpha_k \cdot c N = c \frac{p_k}{q_k} N$. By definition, $N$ is divisible by $q_k$ and hence $n_k$ is a natural number. Further, note that $\sum_k n_k = \sum_k \alpha_k \cdot c N = (\sum_k \alpha_k) \cdot c N  = c N$. The prescribed sequence for the first $c N$ moves is to play action pair $1$ for the first $n_1$ rounds, action pair $2$ for the next $n_2$ rounds and so on until the end of $c N$ rounds. %For the $c N +1$-th round alone, the final action pair is switched out for the action pair indexed $n^2$ that gives maximum possible payoff to the column player. The policy makes arbitrary choices in the remaining $r$ rounds in the event that the follower has cooperated until that point. 
% For all the remaining rounds, the policy prescribes the action pair that maximizes the follower's payoff. If $r= 0$, we rewrite $T = c \cdot N + r$ where $r = N$.

% The intuition behind this ordering is that the policy forces through the more `painful' action pairs for the follower at the beginning while promising rewards for cooperation and threats for defection. This completes the description of the candidate Stackelberg policy.




% \begin{lemma}
% Any best response policy for the follower to the candidate leader policy described above must necessarily follow the prescribed sequence for all $T$ rounds of play.
% \end{lemma}

% NOTE[Natalie]: how are we dealing with tiebreakers? 

% \begin{proof}
% We prove this by induction on the number of rounds that the follower's policy follows the prescribed sequence. The base case is $t =0 $ and is trivially true. Assume that the follower cooperates for the first $t$ rounds. Consider any deviation from the prescribed policy in the $t+1$-th round (where $t+1 <= c N$). The average payoff for the rounds $t+1$ to $c N$ on following the policy is at least the threat level $V$ -- this is because  $\sum_{k} u^2_{k} \alpha_k \ge V$ and we are following a truncated version of the best part of this distribution (from the follower's perspective) when the follower cooperates with the prescribed policy. The average payoff in the final $r >0$ rounds equals the maximum possible payoff $m$. Thus, the total expected payoff is at least $$V \cdot (c N - t) + r \cdot m = V \cdot (c N - t) + m \cdot (r-1) + m$$ Now, consider deviating in the $t+1$-th round. On this single round, the follower may get value as high as $m$. In all remaining $T - t -1 = c \cdot N -t + r - 1$ rounds, the threat will be employed, and thus the follower will get expected payoff no higher than $V$. So the expected payoff is at most
% $$m + V \cdot (c \cdot N - t + r - 1) = V \cdot (c N - t) + V \cdot (r-1) + m$$

% As $m \geq V$, the payoff of obeying the prescribed policy is at least as high as the payoff of deviating from the prescribed policy. So the inductive step holds when $t \leq c \cdot N$. \\

% Finally, consider deviating on any round $t + 1 > c N$. By construction, for all remaining rounds the leader prescribes only the action pair which gives the follower their globally optimal payoff $m$. So, the remaining payoff by obeying is $m \cdot (T - t)$. As $m$ is the maximum payoff for the follower, no other move sequence over the next $T-t$ rounds can get them a higher payoff. Thus, the best response by the follower for all remaining rounds is to obey the prescribed sequence. So the inductive step also holds when $t > c \cdot N$. Therefore, the inductive step always holds, so a best response policy for the follower will always follow the prescribed sequence. \\

% \end{proof}

% \begin{lemma}
% \label{lemma:reach_lp}
% If the follower obeys the prescribed sequence, the resulting payoff for the leader will get a $1 - \frac{1}{c}$ approximation to the optimum value $\opt$ of the LP (recalling that $T = c N + r$).
% \end{lemma}


% \begin{proof}
% In the first $c N$ rounds, the empirical frequencies of the action pair in the resulting transcript (when the follower obeys the prescribed sequence) exactly equals the probability distribution $\alpha$. Therefore, the average payoff of the leader in the first $c N$ rounds equals $\sum_{i,j} u^1_{i,j} \alpha_{i,j}$, which is the objective of the LP for the optimal solution. In the remaining rounds, the difference in the average payoff and the LP's optimum objective is at most $1$ -- therefore, the total payoff is at most $\opt . (c N + r) - r$. Thus, we have a $\frac{\opt . (c N + r) - r}{\opt(c N +r)} = 1 - \frac{r}{c N + r} \ge 1 - \frac{r}{c N} \ge 1 - \frac{1}{c}$- approximation to the LP optimum, where the last inequality comes from $r \le N$.
% \end{proof}


% Putting together Lemmas~\ref{lemma:lp_upper_bd} and \ref{lemma:reach_lp}, our candidate policy is shown to guarantee a payoff to the leader that is a $1 - \frac{1}{c}$-approximation to the value generated by any policy against a rational follower. Further, as $T \rightarrow \infty$, $c \rightarrow \infty$, making our policy optimal in the limit.  


%\begin{lemma}
%The value of the LP upper bounds the value of the best policy, for any T.
%\end{lemma}

\subsection{Open Problems}

\begin{enumerate}
    \item What characterizes games where there is a separation (or no separation) between the Stackelberg policy and repeating the static Stackelberg strategy?
    \item Currently, $N$, our time horizon scaling factor, can have an exponential dependence on the number of actions $n$ and the number of bits used to represent each payoff. Can we do some intelligent rounding of the LP solution to get a polynomial dependence at the cost of some small approximation?
\end{enumerate}
